Binarized Canonical Polyadic Decomposition for Knowledge Graph Completion

Methods based on vector embeddings of knowledge graphs have been actively pursued as a promising approach to knowledge graph completion.However, embedding models generate storage-inefficient representations, particularly when the number of entities and relations, and the dimensionality of the real-valued embedding vectors are large. We present a binarized CANDECOMP/PARAFAC(CP) decomposition algorithm, which we refer to as B-CP, where real-valued parameters are replaced by binary values to reduce model size. Moreover, we show that a fast score computation technique can be developed with bitwise operations. We prove that B-CP is fully expressive by deriving a bound on the size of its embeddings. Experimental results on several benchmark datasets demonstrate that the proposed method successfully reduces model size by more than an order of magnitude while maintaining task performance at the same level as the real-valued CP model.

==> figures/array.tex <==
%\begin{figure}
%\centering
%
%       \scalebox{0.5}{
%       $
%\renewcommand\arraystretch{1.3}
%\begin{blockarray}{ccccccccccccccccccccccccccccccccc}
%	  &1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20&21&22&23&24&25&26&27&28&29&30&31&32\\
%	  \mat{a}_{1:}&
%	  \tikznode{e1}{\Delta}&\Delta&-\Delta&-\Delta&\Delta&-\Delta&\Delta&\tikznode{e2}{-\Delta}&
%	  \tikznode{f1}{\Delta}&\Delta&-\Delta&-\Delta&\Delta&-\Delta&\Delta&\tikznode{f2}{-\Delta}&
%	  \tikznode{a1}{\Delta}&\Delta&-\Delta&-\Delta&\Delta&-\Delta&\Delta&\tikznode{a2}{-\Delta}&
%	  \tikznode{b1}{\Delta}&\Delta&-\Delta&-\Delta&\Delta&-\Delta&\Delta&\tikznode{b2}{-\Delta}\\
%	  \mat{a}_{2:}&
%	  \Delta&-\Delta&\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta&
%	  \Delta&-\Delta&\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta&
%	  \Delta&-\Delta&\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta&
%	  \Delta&-\Delta&\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta\\
%\hline
%	%\mat{b}_{1:}&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?&?\\
%	%\mat{b}_{2:}&
%	%\tikznode{e3}?&?&?&?&?&?&?&\tikznode{e4}{?}&
%	%\tikznode{f3}?&?&?&?&?&?&?&\tikznode{f4}{?}&
%	%\tikznode{a3}{?}&?&?&?&?&?&?&\tikznode{a4}{?}&
%	%\tikznode{b3}{?}&?&?&?&?&?&?&\tikznode{b4}{?}\\
%	\mat{b}_{1:}&
%	\Delta&\Delta&-\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta&
%	\Delta&\Delta&-\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta&
%	\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&-\Delta&-\Delta&
%	\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&-\Delta&-\Delta\\
%	\mat{b}_{2:}&
%	\tikznode{e3}{\Delta}&\Delta&-\Delta&-\Delta&\Delta&\Delta&\Delta&\tikznode{e4}{\Delta}&
%	\tikznode{f3}{\Delta}&\Delta&-\Delta&-\Delta&\Delta&\Delta&\Delta&\tikznode{f4}{\Delta}&
%	\tikznode{a3}{\Delta}&\Delta&-\Delta&-\Delta&\Delta&\Delta&\Delta&\tikznode{a4}{\Delta}&
%	\tikznode{b3}{\Delta}&\Delta&-\Delta&-\Delta&\Delta&\Delta&\Delta&\tikznode{b4}{\Delta}\\
%\hline
%	\mat{c}_{1:}&
%	\tikznode{i1}{\Delta}&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\tikznode{i2}{\Delta}&
%	\tikznode{j1}{\Delta}&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\tikznode{j2}{\Delta}&
%	\tikznode{c1}{\Delta}&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\tikznode{c2}{\Delta}&
%	\tikznode{d1}{-\Delta}&-\Delta&-\Delta&-\Delta&-\Delta&-\Delta&-\Delta&\tikznode{d2}{-\Delta}\\
%	\mat{c}_{2:}&
%	\tikznode{g1}{\Delta}&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\tikznode{g2}{\Delta}&
%	\tikznode{h1}{-\Delta}&-\Delta&-\Delta&-\Delta&-\Delta&-\Delta&-\Delta&\tikznode{h2}{-\Delta}&
%	\tikznode{k1}{\Delta}&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\tikznode{k2}{\Delta}&
%	\tikznode{l1}{\Delta}&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\tikznode{l2}{\Delta}\\
%\end{blockarray}
%$
%\tikz[overlay,remember picture]{
%  \node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(a1) (a2) (a3) (a4)]{}; 
%  \node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(b1) (b2) (b3) (b4)]{}; 
%  \node[draw=kblue,thick, fill=kblue, opacity=0.3, fit=(c1) (c2)]{}; 
%  \node[draw=red,thick, fill=red, opacity=0.3, fit=(d1) (d2)]{}; 
%  \node[draw=kred ,thick, fill=kred, opacity=0.3, fit=(e1) (e2) (e3) (e4)]{}; 
%  \node[draw=kred ,thick, fill=kred, opacity=0.3, fit=(f1) (f2) (f3) (f4)]{}; 
%  \node[draw=kblue,thick, fill=kblue, opacity=0.3, fit=(g1) (g2)]{}; 
%  \node[draw=red,thick, fill=red, opacity=0.3, fit=(h1) (h2)]{}; 
%  \node[draw=kred,thick, fill=kred, opacity=0.3, fit=(i1) (i2)]{}; 
%  \node[draw=kred,thick, fill=kred, opacity=0.3, fit=(j1) (j2)]{}; 
%  \node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(k1) (k2)]{}; 
%  \node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(l1) (l2)]{}; 
%}
%      }
%
%\caption{テンソル$\mat{\mathcal{S}}$の因子行列．部分因子行列が等しいとき
%  同じ色で表している．因子行列\mat{b}はテンソル$\mat{\mathcal{S}}$に依存して定まるため，
%$?$で表している．}
%      \label{fig:array1}
%
%\end{figure}

\begin{figure}
  \centering

  \scalebox{1.3}{
    $
    \renewcommand\arraystretch{1.3}
    \begin{blockarray}{ccccccccccccccccccccccccccccccccc}
	  &1&2&3&4&5&6&7&8\\
      \mat{a}^{(b)}_{1:}&
      \tikznode{a1}{\mat{p}}&\tikznode{a2}{\mat{q}}&\tikznode{b1}{\mat{p}}&\tikznode{b2}{\mat{q}}&
      \tikznode{c1}{\mat{p}}&\tikznode{c2}{\mat{q}}&\tikznode{d1}{\mat{p}}&\tikznode{d2}{\mat{q}}\\
      \mat{a}^{(b)}_{2:}&
      \mat{q}&\mat{p}&\mat{q}&\mat{p}&\mat{q}&\mat{p}&\mat{q}&\mat{p}\\
      \hline
      \mat{b}^{(b)}_{1:}&
      \mat{p}&\mat{p}&\mat{p}&\mat{p}&\mat{r}&\mat{p}&\mat{r}&\mat{p}\\
      \mat{b}^{(b)}_{2:}&
      \mat{p}&\mat{r}&\mat{p}&\mat{r}&
      \tikznode{c3}{\mat{p}}&\tikznode{c4}{\mat{r}}&\tikznode{d3}{\mat{p}}&\tikznode{d4}{\mat{r}}\\
      \hline
      \mat{c}^{(b)}_{1:}&
      \tikznode{a3}{\mat{r}}&\tikznode{a4}{\mat{r}}&\tikznode{b3}{\mat{r}}&\tikznode{b4}{\mat{r}}&
      \tikznode{e1}{\mat{r}}&\tikznode{e2}{\mat{r}}&\tikznode{f1}{-\mat{r}}&\tikznode{f2}{-\mat{r}}\\
      \mat{c}^{(b)}_{2:}&
      \tikznode{g1}{\mat{r}}&\tikznode{g2}{\mat{r}}&\tikznode{h1}{-\mat{r}}&\tikznode{h2}{-\mat{r}}&\tikznode{i1}{\mat{r}}&\tikznode{i2}{\mat{r}}&\tikznode{j1}{\mat{r}}&\tikznode{j2}{\mat{r}}\\
    \end{blockarray}
    $
    \tikz[overlay,remember picture]{
      %\coordinate (e2) at ($(e1)+(-1cm, 0cm)$);
      %\node (x1) at (1, 0);
      %\node (x2) at (0, 0);
      %\draw (-4,0) -- (4,0);
      %\draw (e1.north west) -- (e2.north);
      %\node[draw=kblue, thick, fit=(1a11), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=green, thick, fit=(a1) (a2) (a3) (a4),text width=8mm, inner sep=1]{}; 
      %\node[draw=kred,thick, inner sep=0, fit=(a1) (a2) (a3) (a4)]{}; 
      \node[draw=green,thick, fit=(b1) (b2) (b3) (b4),text width=13mm, inner sep=1]{}; 
      \node[draw=kgreen,thick, fit=(c1) (c2) (c3) (c4),text width=8mm, inner sep=1]{}; 
      \node[draw=kgreen,thick, fit=(d1) (d2) (d3) (d4),text width=13mm, inner sep=1]{}; 
      \node[draw=blue ,thick, fit=(e1) (e2),text width=8mm, inner sep=1, minimum height=3mm]{}; 
      \node[draw=red ,thick, fit=(f1) (f2),text width=13mm, inner sep=1, minimum height=3mm, minimum height=3mm]{}; 
      \node[draw=blue ,thick, fit=(g1) (g2),text width=8mm, inner sep=1, minimum height=3mm, minimum height=3mm]{}; 
      \node[draw=red ,thick, fit=(h1) (h2),text width=13mm, inner sep=1, minimum height=3mm]{}; 
      \node[draw=kgreen, thick, fit=(i1) (i2),text width=8mm, inner sep=1, minimum height=3mm]{}; 
      \node[draw=kgreen,thick, fit=(j1) (j2),text width=13mm, inner sep=1, minimum height=3mm]{}; 
      %\node[draw=kblue,thick, fill=kblue, opacity=0.3, fit=(c1) (c2)]{}; 
      %\node[draw=red,thick, fill=red, opacity=0.3, fit=(d1) (d2)]{}; 
      %\node[draw=kred ,thick, fill=kred, opacity=0.3, fit=(e1) (e2) (e3) (e4)]{}; 
      %\node[draw=kred ,thick, fill=kred, opacity=0.3, fit=(f1) (f2) (f3) (f4)]{}; 
      %\node[draw=kblue,thick, fill=kblue, opacity=0.3, fit=(g1) (g2)]{}; 
      %\node[draw=red,thick, fill=red, opacity=0.3, fit=(h1) (h2)]{}; 
      %\node[draw=kred,thick, fill=kred, opacity=0.3, fit=(i1) (i2)]{}; 
      %\node[draw=kred,thick, fill=kred, opacity=0.3, fit=(j1) (j2)]{}; 
      %\node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(k1) (k2)]{}; 
      %\node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(l1) (l2)]{}; 
    }
  }

  \caption{The binary factor matrices which reconstruct the tensor $\mat{\mathcal{X}}$.
  The part surrounded by the same color indicates that the values are equal.}
    %同じ色で囲まれた部分は値が等しいことを表している．}
  \label{fig:array1}

\end{figure}


==> figures/array2.tex <==
%\begin{figure}
%\centering
%
%
%
%%\begin{columns}
%%\begin{column}{.5\linewidth}
%       \scalebox{1.0}{
%       $
%\renewcommand\arraystretch{1.3}
%%\begin{blockarray}{c|cccccc}
%\begin{blockarray}{ccccccccccccccccc}
%	  &1&2&3&4&5&6&7&8
%	  &&
%	  &1&2&3&4&5&6&7&8\\
%	  \mat{a}_{1:}&
%	  \Delta&\Delta&-\Delta&-\Delta&\Delta&-\Delta&\Delta&-\Delta&&
%	  \mat{a}_{1:}&
%	  \Delta&\Delta&-\Delta&-\Delta&\Delta&-\Delta&\Delta&-\Delta\\
%	  \mat{a}_{2:}&
%	  \Delta&-\Delta&\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta&&
%	  \mat{a}_{2:}&
%	  \Delta&-\Delta&\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta\\
%	  \cline{1-9}
%	  \cline{11-19}
%	\mat{b}_{1:}&
%	\Delta&\Delta&-\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta&&
%	\mat{b}_{1:}&
%	\Delta&\Delta&-\Delta&-\Delta&\Delta&\Delta&-\Delta&-\Delta\\
%	\mat{b}_{2:}&
%	\Delta&\Delta&-\Delta&-\Delta&\Delta&\Delta&\Delta&\Delta&&
%	\mat{b}_{2:}&
%	\Delta&\Delta&-\Delta&-\Delta&\Delta&\Delta&\Delta&\Delta\\
%	  \cline{1-9}
%	  \cline{11-19}
%	\mat{c}_{1:}&
%	\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&&
%	\mat{c}_{1:}&
%	\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta&\Delta\\
%\end{blockarray}
%$
%\tikz[overlay,remember picture]{
%  %\node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(a1) (a2) (a3) (a4)]{}; 
%  %\node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(b1) (b2) (b3) (b4)]{}; 
%  %\node[draw=kblue,thick, fill=kblue, opacity=0.3, fit=(c1) (c2)]{}; 
%  %\node[draw=kred,thick, fill=kred, opacity=0.3, fit=(d1) (d2)]{}; 
%  %\node[draw=red ,thick, fill=red, opacity=0.3, fit=(e1) (e2) (e3) (e4)]{}; 
%  %\node[draw=red ,thick, fill=red, opacity=0.3, fit=(f1) (f2) (f3) (f4)]{}; 
%%\draw (1) -- (2);
%%\draw (ab.south west) -- (ax.south east);
%%\node[fill=blue,opacity=0.3,fit=(s) (3)]{}; 
%}
%      }
%
%\caption{因子行列の1列目から2列目}
%
%\label{fig:array2}
%
%\end{figure}

%\begin{figure}
%  \centering
%
%  \scalebox{1.0}{
%    $
%    %\renewcommand\arraystretch{1.3}
%    \begin{blockarray}{ccc}
%	  &1&2\\
%      \mat{a}_{1:}&
%      \tikznode{a1}{\mat{p}}&\tikznode{a2}{\mat{q}}\\
%      \mat{a}_{2:}&
%      \mat{q}&\mat{p}\\
%      \hline
%      \mat{b}_{1:}&
%      \mat{p}&\mat{p}\\
%      \mat{b}_{2:}&
%      \mat{p}&\mat{r}\\
%      \hline
%      \mat{c}_{1:}&
%      \tikznode{a3}{\mat{r}}&\tikznode{a4}{\mat{r}}\\
%      %\mat{c}_{2:}&
%      %\mat{r}&\mat{r}\\
%    \end{blockarray}
%    $
%    \tikz[overlay,remember picture]{
%      %\coordinate (e2) at ($(e1)+(-1cm, 0cm)$);
%      %\node (x1) at (1, 0);
%      %\node (x2) at (0, 0);
%      %\draw (-4,0) -- (4,0);
%      %\draw (e1.north west) -- (e2.north);
%
%      %\node[draw=kred,thick, fit=(a1) (a2) (a3) (a4)]{}; 
%      %\node[draw=kred,thick, fit=(b1) (b2) (b3) (b4)]{}; 
%      %\node[draw=kgreen,thick, fit=(c1) (c2) (c3) (c4)]{}; 
%      %\node[draw=kgreen,thick, fit=(d1) (d2) (d3) (d4)]{}; 
%    }
%  }
%
%  \caption{因子行列の1列目から2列目}
%  \label{fig:array2}
%
%\end{figure}
\begin{figure}
  \centering

  \scalebox{1.3}{
    $
    %\renewcommand\arraystretch{1.3}
    \begin{blockarray}{ccccccccccccccccccccccccccccccccccccc}
      \multicolumn{3}{c}{$s_{111}$}&&\multicolumn{3}{c}{$s_{121}$}&&\multicolumn{3}{c}{$s_{211}$}
				   &&\multicolumn{3}{c}{$s_{221}$}
				   \\
	  &1&2&&&1&2&&&1&2&&&1&2\\
      \mat{a}_{1:}&
      \tikznode{1a11}{\mat{p}}&\tikznode{1a12}{\mat{q}}&&
      \mat{a}_{1:}&
      \tikznode{2a11}{\mat{p}}&\tikznode{2a12}{\mat{q}}&&
      \mat{a}_{1:}&
      \tikznode{3a11}{\mat{p}}&\tikznode{3a12}{\mat{q}}&&
      \mat{a}_{1:}&
      \tikznode{4a11}{\mat{p}}&\tikznode{4a12}{\mat{q}}\\
      \mat{a}_{2:}&
      \tikznode{1a21}{\mat{q}}&\tikznode{1a22}{\mat{p}}&&
      \mat{a}_{2:}&
      \tikznode{2a21}{\mat{q}}&\tikznode{2a22}{\mat{p}}&&
      \mat{a}_{2:}&
      \tikznode{3a21}{\mat{q}}&\tikznode{3a22}{\mat{p}}&&
      \mat{a}_{2:}&
      \tikznode{4a21}{\mat{q}}&\tikznode{4a22}{\mat{p}}\\
      %\hline
      \mat{b}_{1:}&
      \tikznode{1b11}{\mat{p}}&\tikznode{1b12}{\mat{p}}&&
      \mat{b}_{1:}&
      \tikznode{2b11}{\mat{p}}&\tikznode{2b12}{\mat{p}}&&
      \mat{b}_{1:}&
      \tikznode{3b11}{\mat{r}}&\tikznode{3b12}{\mat{p}}&&
      \mat{b}_{1:}&
      \tikznode{4b11}{\mat{r}}&\tikznode{4b12}{\mat{p}}\\
      \mat{b}_{2:}&
      \tikznode{1b21}{\mat{p}}&\tikznode{1b22}{\mat{p}}&&
      \mat{b}_{2:}&
      \tikznode{2b21}{\mat{p}}&\tikznode{2b22}{\mat{p}}&&
      \mat{b}_{2:}&
      \tikznode{3b21}{\mat{p}}&\tikznode{3b22}{\mat{p}}&&
      \mat{b}_{2:}&
      \tikznode{4b21}{\mat{r}}&\tikznode{4b22}{\mat{p}}\\
      %\hline
      \mat{c}_{1:}&
      \tikznode{1c11}{\mat{r}}&\tikznode{1c12}{\mat{r}}&&
      \mat{c}_{1:}&
      \tikznode{2c11}{\mat{r}}&\tikznode{2c12}{\mat{r}}&&
      \mat{c}_{1:}&
      \tikznode{3c11}{\mat{r}}&\tikznode{3c12}{\mat{r}}&&
      \mat{c}_{1:}&
      \tikznode{4c11}{\mat{r}}&\tikznode{4c12}{\mat{r}}\\
      %\mat{c}_{2:}&
      %\tikznode{a1}{\mat{r}}&\tikznode{a1}{\mat{r}}&\mat{s}&\mat{s}&
      %\mat{r}&\mat{r}&\mat{r}&\mat{r}\\
    \end{blockarray}
    $
    \tikz[overlay,remember picture]{
      %\node[draw=kblue,thick, fill=kblue, opacity=0.3, fit=(1a1)]{};
      %\coordinate (e2) at ($(e1)+(-1cm, 0cm)$);
      %\node (x1) at (1, 0);
      %\node (x2) at (0, 0);
      %\draw (-4,0) -- (4,0);
      %\draw (e1.north west) -- (e2.north);
      %\draw (e1.north west) -- (e2.north);

      %\node[draw=kred,thick, fit=(a1) (a2) (a3) (a4)]{}; 

      \node[draw=kblue, thick, fit=(1a11), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(2a11), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(1a12), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(2a12), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(3a21), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(4a21), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(3a22), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(4a22), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(1b11), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(3b11), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(1b12), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(3b12), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(2b21), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(4b21), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(2b22), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(4b22), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(1c11), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(2c11), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(3c11), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(4c11), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(1c12), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kred, thick, fit=(2c12), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(3c12), text width=3mm, inner sep=0, minimum height=3mm]{};
      \node[draw=kblue, thick, fit=(4c12), text width=3mm, inner sep=0, minimum height=3mm]{};


      %\draw (1a11.north west) -- (1a11.south west) -- (1a11.south east) -- (1a11.north east) -- cycle;
      %\draw (2a11.north west) -- (2a11.south west) -- (2a11.south east) -- (2a11.north east) -- cycle;
      %\draw (3a11.north west) -- (3a11.south west) -- (3a11.south east) -- (3a11.north east) -- cycle;
      %\draw (4a11.north west) -- (4a11.south west) -- (4a11.south east) -- (4a11.north east) -- cycle;
      %\draw (1a12.north west) -- (1a12.south west) -- (1a12.south east) -- (1a12.north east) -- cycle;
      %\draw (2a12.north west) -- (2a12.south west) -- (2a12.south east) -- (2a12.north east) -- cycle;
      %\draw (3a12.north west) -- (3a12.south west) -- (3a12.south east) -- (3a12.north east) -- cycle;
      %\draw (4a12.north west) -- (4a12.south west) -- (4a12.south east) -- (4a12.north east) -- cycle;
      %\draw (1a21.north west) -- (1a21.south west) -- (1a21.south east) -- (1a21.north east) -- cycle;
      %\draw (2a21.north west) -- (2a21.south west) -- (2a21.south east) -- (2a21.north east) -- cycle;
      %\draw (3a21.north west) -- (3a21.south west) -- (3a21.south east) -- (3a21.north east) -- cycle;
      %\draw (4a21.north west) -- (4a21.south west) -- (4a21.south east) -- (4a21.north east) -- cycle;
      %\draw (1a22.north west) -- (1a22.south west) -- (1a22.south east) -- (1a22.north east) -- cycle;
      %\draw (2a22.north west) -- (2a22.south west) -- (2a22.south east) -- (2a22.north east) -- cycle;
      %\draw (3a22.north west) -- (3a22.south west) -- (3a22.south east) -- (3a22.north east) -- cycle;
      %\draw (4a22.north west) -- (4a22.south west) -- (4a22.south east) -- (4a22.north east) -- cycle;
      %\draw (1b11.north west) -- (1b11.south west) -- (1b11.south east) -- (1b11.north east) -- cycle;
      %\draw (2b11.north west) -- (2b11.south west) -- (2b11.south east) -- (2b11.north east) -- cycle;
      %\draw (3b11.north west) -- (3b11.south west) -- (3b11.south east) -- (3b11.north east) -- cycle;
      %\draw (4b11.north west) -- (4b11.south west) -- (4b11.south east) -- (4b11.north east) -- cycle;
      %\draw (1b12.north west) -- (1b12.south west) -- (1b12.south east) -- (1b12.north east) -- cycle;
      %\draw (2b12.north west) -- (2b12.south west) -- (2b12.south east) -- (2b12.north east) -- cycle;
      %\draw (3b12.north west) -- (3b12.south west) -- (3b12.south east) -- (3b12.north east) -- cycle;
      %\draw (4b12.north west) -- (4b12.south west) -- (4b12.south east) -- (4b12.north east) -- cycle;
      %\draw (1b21.north west) -- (1b21.south west) -- (1b21.south east) -- (1b21.north east) -- cycle;
      %\draw (2b21.north west) -- (2b21.south west) -- (2b21.south east) -- (2b21.north east) -- cycle;
      %\draw (3b21.north west) -- (3b21.south west) -- (3b21.south east) -- (3b21.north east) -- cycle;
      %\draw (4b21.north west) -- (4b21.south west) -- (4b21.south east) -- (4b21.north east) -- cycle;
      %\draw (1b22.north west) -- (1b22.south west) -- (1b22.south east) -- (1b22.north east) -- cycle;
      %\draw (2b22.north west) -- (2b22.south west) -- (2b22.south east) -- (2b22.north east) -- cycle;
      %\draw (3b22.north west) -- (3b22.south west) -- (3b22.south east) -- (3b22.north east) -- cycle;
      %\draw (4b22.north west) -- (4b22.south west) -- (4b22.south east) -- (4b22.north east) -- cycle;

      %\draw (1c11.north west) -- (1c11.south west) -- (1c11.south east) -- (1c11.north east) -- cycle;
      %\draw (2c11.north west) -- (2c11.south west) -- (2c11.south east) -- (2c11.north east) -- cycle;
      %\draw (3c11.north west) -- (3c11.south west) -- (3c11.south east) -- (3c11.north east) -- cycle;
      %\draw (4c11.north west) -- (4c11.south west) -- (4c11.south east) -- (4c11.north east) -- cycle;
      %\draw (1c12.north west) -- (1c12.south west) -- (1c12.south east) -- (1c12.north east) -- cycle;
      %\draw (2c12.north west) -- (2c12.south west) -- (2c12.south east) -- (2c12.north east) -- cycle;
      %\draw (3c12.north west) -- (3c12.south west) -- (3c12.south east) -- (3c12.north east) -- cycle;
      %\draw (4c12.north west) -- (4c12.south west) -- (4c12.south east) -- (4c12.north east) -- cycle;
      %\node[draw=kred,thick, fit=(a1) (a2) (a3) (a4)]{}; 
      %\node[draw=kred,thick, fit=(a1) (a2) (a3) (a4)]{}; 
      %\node[draw=kred,thick, fit=(b1) (b2) (b3) (b4)]{}; 
      %\node[draw=kgreen,thick, fit=(c1) (c2) (c3) (c4)]{}; 
      %\node[draw=kgreen,thick, fit=(d1) (d2) (d3) (d4)]{}; 
      %\node[draw=kblue ,thick, fit=(e1) (e2)]{}; 
      %\node[draw=red ,thick, fit=(f1) (f2)]{}; 
      %\node[draw=kblue ,thick, fit=(g1) (g2)]{}; 
      %\node[draw=red ,thick, fit=(h1) (h2)]{}; 
      %\node[draw=kgreen, thick, fit=(i1) (i2)]{}; 
      %\node[draw=kgreen,thick, fit=(j1) (j2)]{}; 
      %\node[draw=kblue,thick, fill=kblue, opacity=0.3, fit=(c1) (c2)]{}; 
      %\node[draw=red,thick, fill=red, opacity=0.3, fit=(d1) (d2)]{}; 
      %\node[draw=kred ,thick, fill=kred, opacity=0.3, fit=(e1) (e2) (e3) (e4)]{}; 
      %\node[draw=kred ,thick, fill=kred, opacity=0.3, fit=(f1) (f2) (f3) (f4)]{}; 
      %\node[draw=kblue,thick, fill=kblue, opacity=0.3, fit=(g1) (g2)]{}; 
      %\node[draw=red,thick, fill=red, opacity=0.3, fit=(h1) (h2)]{}; 
      %\node[draw=kred,thick, fill=kred, opacity=0.3, fit=(i1) (i2)]{}; 
      %\node[draw=kred,thick, fill=kred, opacity=0.3, fit=(j1) (j2)]{}; 
      %\node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(k1) (k2)]{}; 
      %\node[draw=kgreen,thick, fill=kgreen, opacity=0.3, fit=(l1) (l2)]{}; 
    }
  }

  \caption{
    The submatrices which represent the slice $\mat{X}_1$.
    The light blue part shows 
    the submatrices in the term containing $\mat{b}_{j\alpha}$
    , and the orange part shows 
    the submatrices in the term not containing $\mat{b}_{j\alpha}$.
    %スライス$\mat{S}_1$を表す部分二値因子行列．
    %when calculating $s_{111}$，$s_{121}$，$s_{211}$，$s_{221}$,
    %$\mat{b}_{j\alpha}$を含む項(水色の部分)，$\mat{b}_{j\alpha}$
    %を含まない項(橙の部分)を表している．
    }
  \label{fig:array2}

\end{figure}


==> figures/bdist_dist.tex <==
%\begin{figure}[t]
%\centering
%%\includegraphics[height=0.25\textheight]{figures/nation_clustering.png}
%\includegraphics[width=0.85\linewidth]{figures/bdist_path.eps}
%\caption{bdistpath}
%\label{fig:bdist_path}
%\end{figure}
%
\begin{figure}[t]
\centering
\begin{tabular}{c}
\begin{minipage}{0.5\hsize}
\centering
\includegraphics[width=0.95\linewidth]{figures/bdist_dist.eps}
\end{minipage}
\begin{minipage}{0.5\hsize}
\centering
\includegraphics[width=0.95\linewidth]{figures/bdist_path.eps}
\end{minipage}
\end{tabular}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%%% Local Variables:
%%% Mode: LaTeX
%%% TeX-master: "../main"
%%% TeX-engine: xetex
%%% TeX-PDF-mode: t
%%% End:


==> figures/bdist_path.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{c}
\begin{minipage}{0.5\hsize}
\centering
\includegraphics[width=0.85\linewidth]{figures/bdist_dist.eps}
\end{minipage}
\begin{minipage}{0.5\hsize}
\centering
\includegraphics[width=0.85\linewidth]{figures/bdist_path.eps}
\end{minipage}
\end{tabular}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%%% Local Variables:
%%% Mode: LaTeX
%%% TeX-master: "../main"
%%% TeX-engine: xetex
%%% TeX-PDF-mode: t
%%% End:


==> figures/general_factor_matrix.tex <==
\begin{figure}
\begin{eqnarray*}
\scalebox{0.65}{$\displaystyle
  %\begin{array}{c|cccccccc:cccccccc:p{0.8cm}:cccccccc}
  \begin{array}{c|cccccccc|cccccccc|p{0.8cm}|cccccccc}
  \multicolumn{1}{c}{} & 
  \multicolumn{25}{c}{\overbrace{\rule{20cm}{0pt}}^{2N_eN_r}} \\
  \multicolumn{1}{c}{} & 
  \multicolumn{4}{c}{\overbrace{\rule{2.5cm}{0pt}}^{N_e}} &  
  \multicolumn{4}{c}{\overbrace{\rule{3.0cm}{0pt}}^{N_e}} &
  \multicolumn{4}{c}{\overbrace{\rule{2.5cm}{0pt}}^{N_e}} &
  \multicolumn{4}{c}{\overbrace{\rule{3.0cm}{0pt}}^{N_e}} &
  \multicolumn{1}{c}{} & 
  \multicolumn{4}{c}{\overbrace{\rule{2.5cm}{0pt}}^{N_e}} &
  \multicolumn{4}{c}{\overbrace{\rule{3.0cm}{0pt}}^{N_e}} \\
  \bm{a}_{1:}^{(b)} &
	\mat{p} & \mat{q} & \cdots & \mat{q} &
	\mat{p} & \mat{q} & \cdots & \mat{q} &
	\mat{p} & \mat{q} & \cdots & \mat{q} &
	\mat{p} & \mat{q} & \cdots & \mat{q} &
	\multicolumn{1}{c|}{\multirow{4}{*}{$\ldots$}}&
	\mat{p} & \mat{q} & \cdots & \mat{q} &
	\mat{p} & \mat{q} & \cdots & \mat{q} \\
	\bm{a}_{2:}^{(b)} &
	\mat{q} & \mat{p} & \cdots & \mat{q} &
	\mat{q} & \mat{p} & \cdots & \mat{q} &
	\mat{q} & \mat{p} & \cdots & \mat{q} &
	\mat{q} & \mat{p} & \cdots & \mat{q} &
	  & 
	\mat{q} & \mat{p} & \cdots & \mat{q} &
	\mat{q} & \mat{p} & \cdots & \mat{q} \\
	\vdots &
	\vdots & \vdots & \ddots & \vdots & 
	\vdots & \vdots & \ddots & \vdots & 
	\vdots & \vdots & \ddots & \vdots & 
	\vdots & \vdots & \ddots & \vdots &
	       &
	\vdots & \vdots & \ddots & \vdots &
	\vdots & \vdots & \ddots & \vdots \\
	\bm{a}_{N_e:}^{(b)} &
	\mat{q} & \mat{q} & \cdots & \mat{p} &
	\mat{q} & \mat{q} & \cdots & \mat{p} &
	\mat{q} & \mat{q} & \cdots & \mat{p} &
	\mat{q} & \mat{q} & \cdots & \mat{p} &
	  &  
	\mat{q} & \mat{q} & \cdots & \mat{p} &
	\mat{q} & \mat{q} & \cdots & \mat{p} \\
\hline
	\bm{b}_{1:}^{(b)} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\multicolumn{1}{c|}{\multirow{4}{*}{$\ldots$}}&
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi}\\
	\bm{b}_{2:}^{(b)} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	  &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi}\\
	%\cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots \\
	\vdots &
	\vdots & \vdots & \ddots & \vdots & 
	\vdots & \vdots & \ddots & \vdots & 
	\vdots & \vdots & \ddots & \vdots & 
	\vdots & \vdots & \ddots & \vdots &
	       &
	\vdots & \vdots & \ddots & \vdots &
	\vdots & \vdots & \ddots & \vdots \\
	\bm{b}_{N_e:}^{(b)} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	  & 
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi} &
	\mat{\xi} & \mat{\xi} & \cdots & \mat{\xi}\\
\hline
	\bm{c}_{1:}^{(b)} &
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{-r} & \mat{-r} & \cdots & \mat{-r} &
	\multicolumn{1}{c|}{\multirow{4}{*}{$\ldots$}}&
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{-r} & \mat{-r} & \cdots & \mat{-r} \\
	\bm{c}_{2:}^{(b)} &
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{-r} & \mat{-r} & \cdots & \mat{-r} &
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	  &
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{-r} & \mat{-r} & \cdots & \mat{-r} \\
	%\cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots & \cdots \\
	\vdots &
	\vdots & \vdots & \ddots & \vdots & 
	\vdots & \vdots & \ddots & \vdots & 
	\vdots & \vdots & \ddots & \vdots & 
	\vdots & \vdots & \ddots & \vdots &
	       & 
	\vdots & \vdots & \ddots & \vdots &
	\vdots & \vdots & \ddots & \vdots \\
	\bm{c}_{N_r:}^{(b)} &
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{-r} & \mat{-r} & \cdots & \mat{-r} &
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{-r} & \mat{-r} & \cdots & \mat{-r} &
	  & 
	\mat{r} & \mat{r} & \cdots & \mat{r} &
	\mat{r} & \mat{r} & \cdots & \mat{r} \\
\end{array}
$}
\end{eqnarray*}
\caption{The binary factor matrices which represent tensor $\mat{\mathcal{X}}$.
$\mat{\xi}$ represents either $\mat{p}$ or $\mat{r}$.}
\label{fig:general_factor_matrix}
\end{figure}


==> tables/freebase_music.tex <==
\begin{table}[t]
  \centering
  %\small
  %\caption{Results on the Freebase-music dataset.}
  \label{tab:ldata}
  \begin{tabular}{lcccccc}
  \toprule
		 & Entity& Relation & Train & Valid & Test \\\midrule
	  freebase\_music    & 3,025,684         & 138 & 18,460,832 &1000&1000\\
  %CP~$(D=200)$   & 89.2     & 4.8GB \\
  %{\bf B-CP}~$(D=400)$ & {\bf 92.8}     & {\bf 0.3GB} \\
  \bottomrule
  \end{tabular} 
  %\scalebox{1.0}{
  %\begin{tabular}{lrrrrrrrrr}
  %  \toprule
  %  & & &        & Base    &        &         & \multicolumn{2}{c}{Path}        & \\
  %  & $|\mathcal{E}|$ & $|\mathcal{R}|$ & \#train & \#valid & \#test & \#train & \#valid   & \#test & \#test-uniq \\
  %  % \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}
  %  \cmidrule(lr){1-10}
  %  WN18  & & & 141,442 & 5,000 & 5,000 \\%& 5,760,450 & 10,000 & 10,000 & 13,133 \\
  %  FB15k & & & 483,142 & 50,000 & 59,071 \\%& 7,861,321 & 30,000 & 30,000 & 59,586 \\
  %  YAGO3-10 & \\
  %  \bottomrule
  %\end{tabular}
  %}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%% Local Variables:
%% Mode: LaTeX
%% TeX-master: "../main"
%% TeX-PDF-mode: t
%% End:



==> tables/ldataset.tex <==
\begin{table}[t]
  \centering
  \mytablefont
  \caption{Results on the Freebase-music dataset.}
  \label{tab:ldata}
  \begin{tabular}{lcccc}
  \toprule
                 & Accuracy & Model size \\\midrule
  CP~$(D=15)$    & 50.3         & 0.4GB \\
  CP~$(D=200)$   & 89.2     & 4.8GB \\
  {\bf B-CP}~$(D=400)$ & {\bf 92.8}     & {\bf 0.3GB} \\
  \bottomrule
  \end{tabular} 
  %\scalebox{1.0}{
  %\begin{tabular}{lrrrrrrrrr}
  %  \toprule
  %  & & &        & Base    &        &         & \multicolumn{2}{c}{Path}        & \\
  %  & $|\mathcal{E}|$ & $|\mathcal{R}|$ & \#train & \#valid & \#test & \#train & \#valid   & \#test & \#test-uniq \\
  %  % \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}
  %  \cmidrule(lr){1-10}
  %  WN18  & & & 141,442 & 5,000 & 5,000 \\%& 5,760,450 & 10,000 & 10,000 & 13,133 \\
  %  FB15k & & & 483,142 & 50,000 & 59,071 \\%& 7,861,321 & 30,000 & 30,000 & 59,586 \\
  %  YAGO3-10 & \\
  %  \bottomrule
  %\end{tabular}
  %}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%% Local Variables:
%% Mode: LaTeX
%% TeX-master: "../main"
%% TeX-engine: xetex
%% TeX-PDF-mode: t
%% End:



==> tables/results2.tex <==
\begin{table*}[tb]
  \mytablefont
  \caption{KGC results on WN18RR and FB15k-237: Filtered MRR and Hits@$\{1,3,10\}$ (\%).
      * indicates the results transcribed from~\cite{conve}.}
  \label{tab:results_2}
  \centering
    \begin{tabular}{lccccccccccccccccc}
      \toprule
      & &\multicolumn{4}{c}{WN18RR}   & \multicolumn{4}{c}{FB15k-237} & \multicolumn{4}{c}{WN18}
      & \multicolumn{4}{c}{FB15k} \\
      \cmidrule(lr){3-6}\cmidrule(lr){7-10} \cmidrule(lr){11-14}\cmidrule(lr){15-18}
      & &\multirow{2}{*}{MRR} & \multicolumn{3}{c}{Hits@} & \multirow{2}{*}{MRR} & \multicolumn{3}{c}{Hits@} &\multirow{2}{*}{MRR} & \multicolumn{3}{c}{Hits@} & \multirow{2}{*}{MRR} & \multicolumn{3}{c}{Hits@} \\
      \cmidrule(lr){4-6}\cmidrule(lr){8-10}\cmidrule(lr){12-14}\cmidrule(lr){16-18}
      Models    & Model Size(MB) &      & 1    & 3    & 10   &      & 1    & 3    & 10  &      & 1    & 3    & 10   &      & 1    & 3    & 10 \\\midrule
      TransE*  & -- & -- & -- & -- & -- & -- & -- & -- & -- & 45.4 & 8.9  & 82.3 & 93.4 & 38.0 & 23.1 & 47.2 & 64.1  \\
      DistMult* & 32& 43.0 & 39.0 & 44.0 & 49.0 & 24.1 & 15.5 & 26.3 & 41.9 & 82.2 & 72.8 & 91.4 & 93.6 & 65.4 & 54.6 & 73.3 & 82.4  \\
      HolE*    & -- & -- & -- & -- & -- & -- & -- & -- & -- & 93.8 & 93.0 & 94.5 & 94.9 & 52.4 & 40.2 & 61.3 & 73.9  \\
      ANALOGY**& -- & -- & -- & -- & -- & -- & -- & -- & -- & 94.2 & 93.9 & 94.4 & 94.7 & 72.5 & 64.6 & {\bf 78.5} & {\bf 85.4}  \\
      CP***    & -- & -- & -- & -- & -- & -- & -- & -- & -- & 94.2 & 93.9 & 94.4 & 94.7 & 72.7 & 66.0 & 77.3 & 83.9 \\
      ComplEx*  & 64& 44.0 & 41.0 & 46.0 & 51.0 & 24.7 & 15.8 & 27.5 & 42.8 & 94.1 & 93.6 & 94.5 & 94.7 & 69.2 & 59.9 & 75.9 & 84.0  \\
      R-GCN*    & -- & --   & --   & --   & --   & 24.8 & 15.3 & 25.8 & 41.7 &-- &-- & -- & --& --& -- & -- & --\\
      ConvE*    & 32 & 43.0 & 40.0 & 44.0 & 52.0 & {\bf 32.5} & {\bf 23.7} & {\bf 35.6} & {\bf 50.1} & 94.3 & 93.5 & 94.6 & {\bf 95.6} & 65.7 & 55.8 & 72.3 & 83.1  \\\midrule
      VQ-CP(D=200) & 2 & 38.0 & -- & -- & 44.0 & 23.0 & -- & -- & 42.0 & -- & -- & -- & -- & -- & -- & -- & -- \\
      VQ-CP(D=500) & 5 & 45.0 & -- & -- & 52.0 & 29.2 & -- & -- & 46.1 & -- & -- & -- & -- & -- & -- & -- & -- \\
      CP(D=15) & 5 & 40.0 & -- & -- & 47.0 & 24.1 & -- & -- & 41.9 & -- & -- & -- & -- & -- & -- & -- & -- \\
      CP(D=50) & 16 & 43.0 & -- & -- & 49.0 & 24.8 & -- & -- & 43.0 & -- & -- & -- & -- & -- & -- & -- & -- \\
      CP ($D=200$)       & 64 & 44.0 & 42.0 & 46.0 & 51.0 & 29.0 & 19.8 & 32.2 & 47.9 & 94.2 & 93.9 & 94.5 & 94.7 & 71.9 & 66.2 & 75.2 & 82.0 \\
      {\bf B-CP} ($D=200$) & 2& 45.0 & 43.0 & 46.0 & 50.0 & 27.8 & 19.4 & 30.4 & 44.6 & 90.1 & 88.1 & 91.8 & 93.3 & 69.5 & 61.1 & 76.0 & 83.5 \\
      {\bf B-CP} ($D=400$) & 4 & 45.0 & 43.0 & 46.0 & 52.0 & 29.2 & 20.8 & 31.8 & 46.1 & 94.5 & 94.1 & 94.8 & 95.0 & 72.2 & 66.3 & 77.5 & 84.2 \\
      {\bf B-CP} ($D=500$) & 5 & 45.0 & -- & -- & 52.0 & 29.2 & -- & -- & 46.1 & -- & -- & -- & -- & -- & -- & -- & -- \\
      {\bf B-CP} ($D=300\times3$) & -- & {\bf 48.0} & {\bf 45.0} & {\bf 49.0} & {\bf 53.0} & 30.3 & 21.4 & 33.3 & 48.2 & {\bf 94.6} & {\bf 94.2} & {\bf 95.0} & 95.3 & {\bf 72.9} & {\bf 66.5} & 77.7 & 84.9 \\\bottomrule
      %{\bf B-CP} ($D=400\times3$) \\\bottomrule
    \end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%% Local Variables:
%% Mode: LaTeX
%% TeX-master: "../main"
%% TeX-engine: xetex
%% TeX-PDF-mode: t
%% End:



==> tables/results_comp.tex <==
\begin{table*}[tb]
  \mytablefont
  \caption{Results on WN18RR and FB15k-237 with varying embedding dimensions.}
  \label{tab:results_comp}
  \centering
    \begin{tabular}{lrrcc}
       \toprule
       \multirow{2}{*}{Model} & \multirow{2}{*}{Bits per entity} & \multirow{2}{*}{Bits per relation} & \multicolumn{2}{c}{MRR} \\
       & & & WN18RR & FB15k-237 \\\midrule
       DistMult* ($D=200$) & 6,400 & 6,400 & 43.0 & 24.1 \\
       ComplEx* ($D=200$) & 12,800 & 12,800 & 44.0 & 24.7 \\
       ConvE* ($D=200$)  & 6,400 & 6,400 & 43.0 & {\bf 32.5} \\\midrule
       CP ($D=15$)   & 960 & 480 & 40.0 & 22.0 \\
       CP ($D=50$)   & 3,200 & 1,600 & 43.0 & 24.8 \\
       CP ($D=200$)  & 12,800 & 6,400 & 44.0 & 29.0 \\
       CP ($D=500$)  & 32,000 & 16,000 & 43.0 & 29.2 \\
       %CP ($D=300\times3$)  & 57,600 & 28,800 &  &  \\ 
       VQ-CP ($D=200$) & 400 & 200 & 36.0 & 8.7 \\
       VQ-CP ($D=500$)  & 1,000 & 500 & 36.0 & 8.3 \\\midrule
       {\bf B-CP} ($D=100$) & 200 & 100 & 38.0 & 23.2 \\
       {\bf B-CP} ($D=200$) & 400 & 200 & 45.0 & 27.8 \\
       {\bf B-CP} ($D=300$) & 600 & 300 & 46.0 & 29.0 \\
       {\bf B-CP} ($D=400$) & 800 & 400 & 45.0 & 29.2 \\
       {\bf B-CP} ($D=500$) & 1,000 & 500 & 45.0 & 29.1 \\
       {\bf B-CP} ($D=300\times3$) & 1,800 & 900 & {\bf 48.0} & 30.3 \\\bottomrule
    \end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%% Local Variables:
%% Mode: LaTeX
%% TeX-master: "../main"
%% TeX-engine: xetex
%% TeX-PDF-mode: t
%% End:


